An Empirical Investigation into Benchmarking Model Multiplicity for Trustworthy Machine Learning: A Case Study on Image Classification

Deep learning models have proven to be highly successful. Yet, their over-parameterization gives rise to model multiplicity, a phenomenon in which multiple models achieve similar performance but exhibit distinct underlying behaviours. This multiplicity presents a significant challenge and necessitates additional specifications in model selection to prevent unexpected failures during deployment. While prior studies have examined these concerns, they focus on individual metrics in isolation, making it difficult to obtain a comprehensive view of multiplicity in trustworthy machine learning. Our work stands out by offering a one-stop empirical benchmark of multiplicity across various dimensions of model design and its impact on a diverse set of trustworthy metrics. In this work, we establish a consistent language for studying model multiplicity by translating several trustworthy metrics into accuracy under appropriate interventions. We also develop a framework, which we call multiplicity sheets, to benchmark multiplicity in various scenarios. We demonstrate the advantages of our setup through a case study in image classification and provide actionable insights into the impact and trends of different hyperparameters on model multiplicity. Finally, we show that multiplicity persists in deep learning models even after enforcing additional specifications during model selection, highlighting the severity of over-parameterization. The concerns of under-specification thus remain, and we seek to promote a more comprehensive discussion of multiplicity in trustworthy machine learning.

==> sections/decision_boundary.tex <==
\section{Prediction Mismatch and Decision Boundary}

In the previous section, we explored the concept of multiplicity in deep learning models, focusing on the impact of various axes such as random seeds, hyperparameters, architecture, and pre-trained weights on model performance. In this section, we delve deeper into raw multiplicity by examining the predictive behavior of different models. We aim to illustrate that the issue of multiplicity extends beyond mere variations in model accuracy and encompasses the diversity of predictions and decision boundaries, even among models with similar performance levels.

\paragraph{Prediction Mismatch:}
To understand the extent of multiplicity in deep learning models, we begin by analyzing the raw predictions of several models on a common test dataset. Figure 1 showcases the results, revealing how the predictions of different models with similar accuracy may exhibit significant variations. Despite achieving comparable accuracy levels, these models can arrive at distinct predictions for individual data points, highlighting the inherent diversity in their learned representations.

\paragraph{Decision Boundaries:}
In addition to examining raw predictions, we assess the decision boundaries of these models using the method described in ABC et al. This approach provides a metric for measuring the similarity between decision boundaries, allowing us to discern the degree of diversity among model architectures. Figure 2 visualizes the decision boundaries, illustrating the considerable variability across models, even those with similar accuracy scores.

The central objective of this section is to underscore that multiplicity goes beyond what is apparent from a model's accuracy alone. While accuracy serves as a standard metric for evaluating model performance, it fails to capture the intricate variations in predictions and decision boundaries that exist among models. The raw multiplicity observed in this study reveals the nuanced and diverse nature of deep learning models, even when they exhibit similar accuracy levels.
Even when assessing each trustworthy machine learning metric independently, we may not perceive the full extent of multiplicity due to the underlying under-specification issue.

As we move forward to discuss multiple trustworthy machine learning metrics in a later section, we will encounter the persistence of under-specification and multiplicity. The findings in this section demonstrate that deep learning models, though achieving comparable accuracy, can exhibit remarkably different behaviors and decision-making processes. This inherent diversity poses a continuing challenge in reliably evaluating model trustworthiness and comprehending the underlying factors influencing model predictions.

In conclusion, this section highlights the raw multiplicity in the predictive behavior of different deep learning models. By examining raw predictions and decision boundaries, we uncover the significant variations among models, even those with similar accuracy levels. The presence of multiplicity beyond accuracy and the lingering issue of under-specification emphasize the need for a more comprehensive and nuanced approach to evaluate model performance and trustworthiness. In the subsequent sections, we will further investigate the impact of multiplicity on various trustworthy machine learning metrics, seeking a more holistic understanding of model behavior and the underlying causes of this diversity.
